Certifiable Relative Pose Estimation

In this paper we present the first fast optimality certifier for the non-minimal version of the Relative Pose problem for calibrated cameras from epipolar constraints. The proposed certifier is based on Lagrangian duality and relies on a novel closed-form expression for dual points. We also leverage an efficient solver that performs local optimization on the manifold of the original problem's non-convex domain. The optimality of the solution is then checked via our novel fast certifier. The extensive conducted experiments demonstrate that, despite its simplicity, this certifiable solver performs excellently on synthetic data, repeatedly attaining the (certified \textit{a posteriori}) optimal solution and shows a satisfactory performance on real data.

==> biblio.tex <==
@article{Zhao2019,
  title={An Efficient Solution to Non-Minimal Case Essential Matrix Estimation},
  author={Zhao, Ji},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2020},
  doi = {10.1109/TPAMI.2020.3030161},
  publisher={IEEE}
}

@article{gomez2019pl,
  title={PL-SLAM: A stereo SLAM system through the combination of points and line segments},
  author={Gomez-Ojeda, Ruben and Moreno, Francisco-Angel and Zu{\~n}iga-No{\"e}l, David and Scaramuzza, Davide and Gonzalez-Jimenez, Javier},
  journal={IEEE Transactions on Robotics},
  volume={35},
  number={3},
  pages={734--746},
  year={2019},
  publisher={IEEE}
}

@article{ozyecsil2017survey,
  title={A survey of structure from motion*.},
  author={{\"O}zye{\c{s}}il, Onur and Voroninski, Vladislav and Basri, Ronen and Singer, Amit},
  journal={Acta Numerica},
  volume={26},
  pages={305--364},
  year={2017},
  publisher={Cambridge University Press}
}

@article{wachsmuth2013licq,
  title={On LICQ and the uniqueness of Lagrange multipliers},
  author={Wachsmuth, Gerd},
  journal={Operations Research Letters},
  volume={41},
  number={1},
  pages={78--80},
  year={2013},
  publisher={Elsevier}
}

@article{fischler1981random,
  title={Random sample consensus: a paradigm for model fitting with applications to image analysis and automated cartography},
  author={Fischler, Martin A and Bolles, Robert C},
  journal={Communications of the ACM},
  volume={24},
  number={6},
  pages={381--395},
  year={1981},
  publisher={ACM New York, NY, USA}
}

@article{yang2020teaser,
  title={TEASER: Fast and Certifiable Point Cloud Registration},
  author={Yang, Heng and Shi, Jingnan and Carlone, Luca},
  journal={arXiv preprint arXiv:2001.07715},
  year={2020}
}

@inproceedings{bay2006surf,
  title={Surf: Speeded up robust features},
  author={Bay, Herbert and Tuytelaars, Tinne and Van Gool, Luc},
  booktitle={European conference on computer vision},
  pages={404--417},
  year={2006},
  organization={Springer}
}
@article{longuet1981computer,
  title={A computer algorithm for reconstructing a scene from two projections},
  author={Longuet-Higgins, H Christopher},
  journal={Nature},
  volume={293},
  number={5828},
  pages={133--135},
  year={1981},
  publisher={Springer}
}

@inproceedings{triggs1999bundle,
  title={Bundle adjustment—a modern synthesis},
  author={Triggs, Bill and McLauchlan, Philip F and Hartley, Richard I and Fitzgibbon, Andrew W},
  booktitle={International workshop on vision algorithms},
  pages={298--372},
  year={1999},
  organization={Springer}
}

@article{mur2015orb,
  title={ORB-SLAM: a versatile and accurate monocular SLAM system},
  author={Mur-Artal, Raul and Montiel, Jose Maria Martinez and Tardos, Juan D},
  journal={IEEE transactions on robotics},
  volume={31},
  number={5},
  pages={1147--1163},
  year={2015},
  publisher={IEEE}
}

@article{stewenius2006recent,
  title={Recent developments on direct relative orientation},
  author={Stewenius, Henrik and Engels, Christopher and Nist{\'e}r, David},
  journal={ISPRS Journal of Photogrammetry and Remote Sensing},
  volume={60},
  number={4},
  pages={284--294},
  year={2006},
  publisher={Elsevier}
}

@article{nister2004efficient,
  title={An efficient solution to the five-point relative pose problem},
  author={Nist{\'e}r, David},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={26},
  number={6},
  pages={756--770},
  year={2004},
  publisher={IEEE}
}

@article{rosen2019se,
  title={SE-Sync: A certifiably correct algorithm for synchronization over the special Euclidean group},
  author={Rosen, David M and Carlone, Luca and Bandeira, Afonso S and Leonard, John J},
  journal={The International Journal of Robotics Research},
  volume={38},
  number={2-3},
  pages={95--125},
  year={2019},
  publisher={Sage Publications Sage UK: London, England}
}


@article{bandeira2016note,
  title={A note on probably certifiably correct algorithms},
  author={Bandeira, Afonso S},
  journal={Comptes Rendus Mathematique},
  volume={354},
  number={3},
  pages={329--333},
  year={2016},
  publisher={Elsevier}
}

@article{yamashita2003implementation,
  title={Implementation and evaluation of SDPA 6.0 (semidefinite programming algorithm 6.0)},
  author={Yamashita, Makoto and Fujisawa, Katsuki and Kojima, Masakazu},
  journal={Optimization Methods and Software},
  volume={18},
  number={4},
  pages={491--505},
  year={2003},
  publisher={Taylor \& Francis}
}

@article{briales2017cartan,
  title={Cartan-sync: Fast and global SE (d)-synchronization},
  author={Briales, Jesus and Gonzalez-Jimenez, Javier},
  journal={IEEE Robotics and Automation Letters},
  volume={2},
  number={4},
  pages={2127--2134},
  year={2017},
  publisher={IEEE}
}

@mastersthesis{ding2007efficient,
  title={On efficient semidefinite relaxations for quadratically constrained quadratic programming},
  author={Ding, Yichuan},
  year={2007},
  school={University of Waterloo}
}


@book{nocedal2006numerical,
  title={Numerical optimization},
  author={Nocedal, Jorge and Wright, Stephen},
  year={2006},
  publisher={Springer Science \& Business Media}
}

@article{hartley1997defense,
  title={In defense of the eight-point algorithm},
  author={Hartley, Richard I},
  journal={IEEE Transactions on pattern analysis and machine intelligence},
  volume={19},
  number={6},
  pages={580--593},
  year={1997},
  publisher={IEEE}
}


@article{jibrin2007identifying,
  title={Identifying redundant linear constraints in systems of linear matrix inequality constraints},
  author={Jibrin, Shafiu and Stover, Daniel},
  journal={Journal of Interdisciplinary Mathematics},
  volume={10},
  number={5},
  pages={601--617},
  year={2007},
  publisher={Taylor \& Francis}
}


@article{faugeras1990motion,
  title={Motion from point matches: multiplicity of solutions},
  author={Faugeras, Olivier D and Maybank, Steve},
  journal={International Journal of Computer Vision},
  volume={4},
  number={3},
  pages={225--246},
  year={1990},
  publisher={Springer}
}

@inproceedings{kukelova2008polynomial,
  title={Polynomial Eigenvalue Solutions to the 5-pt and 6-pt Relative Pose Problems.},
  author={Kukelova, Zuzana and Bujnak, Martin and Pajdla, Tomas},
  booktitle={BMVC},
  volume={2},
  number={5},
  pages={2008},
  year={2008}
}

@inproceedings{kukelova2007two,
  title={Two minimal problems for cameras with radial distortion},
  author={Kukelova, Zuzana and Pajdla, Tomas},
  booktitle={2007 IEEE 11th International Conference on Computer Vision},
  pages={1--8},
  year={2007},
  organization={IEEE}
}


@inproceedings{schops2017multi,
  title={A multi-view stereo benchmark with high-resolution images and multi-camera videos},
  author={Schops, Thomas and Schonberger, Johannes L and Galliani, Silvano and Sattler, Torsten and Schindler, Konrad and Pollefeys, Marc and Geiger, Andreas},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={3260--3269},
  year={2017}
}

@inproceedings{lui2013iterative,
  title={An Iterative 5-pt Algorithm for Fast and Robust Essential Matrix Estimation.},
  author={Lui, Vincent and Drummond, Tom},
  booktitle={BMVC},
  year={2013}
}

@inproceedings{yang2014optimal,
  title={Optimal essential matrix estimation via inlier-set maximization},
  author={Yang, Jiaolong and Li, Hongdong and Jia, Yunde},
  booktitle={European Conference on Computer Vision},
  pages={111--126},
  year={2014},
  organization={Springer}
}

@inproceedings{briales2016fast,
  title={Fast global optimality verification in 3D SLAM},
  author={Briales, Jesus and Gonzalez-Jimenez, Javier},
  booktitle={2016 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={4630--4636},
  year={2016},
  organization={IEEE}
}

@article{helmke2007essential,
  title={Essential matrix estimation using Gauss-Newton iterations on a manifold},
  author={Helmke, Uwe and H{\"u}per, Knut and Lee, Pei Yean and Moore, John},
  journal={International Journal of Computer Vision},
  volume={74},
  number={2},
  pages={117--136},
  year={2007},
  publisher={Springer}
}

@inproceedings{kneip2013direct,
  title={Direct optimization of frame-to-frame rotation},
  author={Kneip, Laurent and Lynen, Simon},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2352--2359},
  year={2013}
}

@article{ma2001optimization,
  title={Optimization criteria and geometric algorithms for motion and structure estimation},
  author={Ma, Yi and Ko{\v{s}}eck{\'a}, Jana and Sastry, Shankar},
  journal={International Journal of Computer Vision},
  volume={44},
  number={3},
  pages={219--249},
  year={2001},
  publisher={Springer}
}

@inproceedings{hartley2007global,
  title={Global optimization through searching rotation space and optimal estimation of the essential matrix},
  author={Hartley, Richard I and Kahl, Fredrik},
  booktitle={2007 IEEE 11th International Conference on Computer Vision},
  pages={1--8},
  year={2007},
  organization={IEEE}
}

@inproceedings{botterill2011refining,
  title={Refining essential matrix estimates from RANSAC},
  author={Botterill, Tom and Mills, Steven and Green, Richard},
  booktitle={Proceedings Image and Vision Computing New Zealand},
  pages={1--6},
  year={2011}
}

@inproceedings{song2013parallel,
  title={Parallel, real-time monocular visual odometry},
  author={Song, Shiyu and Chandraker, Manmohan and Guest, Clark C},
  booktitle={2013 ieee international conference on robotics and automation},
  pages={4698--4705},
  year={2013},
  organization={IEEE}
}

@book{absil2009optimization,
  title={Optimization algorithms on matrix manifolds},
  author={Absil, P-A and Mahony, Robert and Sepulchre, Rodolphe},
  year={2009},
  publisher={Princeton University Press}
}

@inproceedings{dubbelman2012manifold,
  title={Manifold statistics for essential matrices},
  author={Dubbelman, Gijs and Dorst, Leo and Pijls, Henk},
  booktitle={European Conference on Computer Vision},
  pages={531--544},
  year={2012},
  organization={Springer}
}

@article{tron2017space,
  title={The space of essential matrices as a Riemannian quotient manifold},
  author={Tron, Roberto and Daniilidis, Kostas},
  journal={SIAM Journal on Imaging Sciences},
  volume={10},
  number={3},
  pages={1416--1445},
  year={2017},
  publisher={SIAM}
}

@article{toh1999sdpt3,
  title={SDPT3—a MATLAB software package for semidefinite programming, version 1.3},
  author={Toh, Kim-Chuan and Todd, Michael J and T{\"u}t{\"u}nc{\"u}, Reha H},
  journal={Optimization methods and software},
  volume={11},
  number={1-4},
  pages={545--581},
  year={1999},
  publisher={Taylor \& Francis}
}

@incollection{gb08,
  author    = {Michael Grant and Stephen Boyd},
  title     = {Graph implementations for nonsmooth convex programs},
  booktitle = {Recent Advances in Learning and Control},
  series    = {Lecture Notes in Control and Information Sciences},
  editor    = {V. Blondel and S. Boyd and H. Kimura},
  publisher = {Springer-Verlag Limited},
  pages     = {95--110},
  year      = 2008
  }
  % url      = {http://stanford.edu/~boyd/graph_dcp.html}
%}

@book{hartley2003multiple,
  title={Multiple view geometry in computer vision},
  author={Hartley, Richard and Zisserman, Andrew},
  year={2003},
  publisher={Cambridge university press}
}

@book{ma2012invitation,
  title={An invitation to 3-d vision: from images to geometric models},
  author={Ma, Yi and Soatto, Stefano and Kosecka, Jana and Sastry, S Shankar},
  volume={26},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@inproceedings{zheng2013revisiting,
  title={Revisiting the pnp problem: A fast, general and optimal solution},
  author={Zheng, Yinqiang and Kuang, Yubin and Sugimoto, Shigeki and Astrom, Kalle and Okutomi, Masatoshi},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2344--2351},
  year={2013}
}


@inproceedings{cheng2015convex,
  title={A convex optimization approach to robust fundamental matrix estimation},
  author={Cheng, Yongfang and Lopez, Jose A and Camps, Octavia and Sznaier, Mario},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={2170--2178},
  year={2015}
}

@article{ma2010semidefinite,
  title={Semidefinite relaxation of quadratic optimization problems and applications},
  author={Ma, Wing-Kin Ken},
  journal={IEEE Signal Processing Magazine},
  volume={1053},
  number={5888/10},
  year={2010},
  publisher={Citeseer}
}

@article{manopt,
  author  = {Boumal, N. and Mishra, B. and Absil, P.-A. and Sepulchre, R.},
  title   = {{M}anopt, a {M}atlab Toolbox for Optimization on Manifolds},
  journal = {Journal of Machine Learning Research},
  year    = {2014},
  volume  = {15},
  pages   = {1455--1459},
  url     = {http://www.manopt.org}
}

@book{meyer2000matrix,
  title={Matrix analysis and applied linear algebra},
  author={Meyer, Carl D},
  volume={71},
  year={2000},
  publisher={Siam}
}

@article{tian2019block,
  title={Block-Coordinate Descent on the Riemannian Staircase for Certifiably Correct Distributed Rotation and Pose Synchronization},
  author={Tian, Yulun and Khosoussi, Kasra and How, Jonathan P},
  journal={arXiv preprint arXiv:1911.03721},
  year={2019}
}

@inproceedings{eriksson2018rotation,
  title={Rotation averaging and strong duality},
  author={Eriksson, Anders and Olsson, Carl and Kahl, Fredrik and Chin, Tat-Jun},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={127--135},
  year={2018}
}

@inproceedings{carlone2015duality,
  title={Duality-based verification techniques for 2D SLAM},
  author={Carlone, Luca and Dellaert, Frank},
  booktitle={2015 IEEE international conference on robotics and automation (ICRA)},
  pages={4589--4596},
  year={2015},
  organization={IEEE}
}
@inproceedings{carlone2015lagrangian,
  title={Lagrangian duality in 3D SLAM: Verification techniques and optimal solutions},
  author={Carlone, Luca and Rosen, David M and Calafiore, Giuseppe and Leonard, John J and Dellaert, Frank},
  booktitle={2015 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={125--132},
  year={2015},
  organization={IEEE}
}

@inproceedings{briales2018certifiably,
  title={A certifiably globally optimal solution to the non-minimal relative pose problem},
  author={Briales, Jesus and Kneip, Laurent and Gonzalez-Jimenez, Javier},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={145--154},
  year={2018}
}

@book{boyd2004convex,
  title={Convex optimization},
  author={Boyd, Stephen and Vandenberghe, Lieven},
  year={2004},
  publisher={Cambridge university press}
}

@article{sturm1999using,
  title={Using SeDuMi 1.02, a MATLAB toolbox for optimization over symmetric cones},
  author={Sturm, Jos F},
  journal={Optimization methods and software},
  volume={11},
  number={1-4},
  pages={625--653},
  year={1999},
  publisher={Taylor \& Francis}
}
